Quasars at intermediate redshift are not special; but they are often satellites

Understanding the links between the activity of supermassive black holes (SMBH) at the centres of galaxies and their host dark matter haloes is a key question in modern astrophysics. The final data release of the SDSS-IV eBOSS provides the largest contemporary spectroscopic sample of galaxies and QSOs. Using this sample and covering the redshift interval $z=0.7-1.1$, we have measured the clustering properties of the eBOSS QSOs, Emission Line Galaxies (ELGs) and Luminous Red Galaxies (LRGs). We have also measured the fraction of QSOs as a function of the overdensity defined by the galaxy population. Using these measurements, we investigate how QSOs populate and sample the galaxy population, and how the host dark-matter haloes of QSOs sample the underlying halo distribution. We find that the probability of a galaxy hosting a QSO is independent of the host dark matter halo mass of the galaxy. We also find that about 60\% of eBOSS QSOs are hosted by LRGs and about 20-40\% of QSOs are hosted by satellite galaxies. We find a slight preference for QSOs to populate satellite galaxies over central galaxies. This is connected to the host halo mass distribution of different types of galaxies. Based on our analysis, QSOs should be hosted by a very broad distribution of haloes, and their occurrence should be modulated only by the efficiency of galaxy formation processes.

==> Tex/analysis.tex <==
\section{Analysis}
\label{sec:analysis}

\begin{table}
    \centering
    \caption{List of parameters and priors in our mcmc analysis}
    \begin{tabular}{p{1.2cm} p{4.5cm} p{1.2cm}} \hline\hline
    {\bf Parameters} &  {\bf comment} & {\bf prior} \\ [0.5ex] \hline\hline
     $f_{\rm on}(M_{i}^{\rm knot})$ & probability of turn-on for $i=0-7$ at halo masses given in table \ref{tab:par-model}. & 0-1  \\ [0.9ex]\hdashline \\
     $f_{\rm LRG}$ & fraction of LRG hosting QSO. & 0-1  \\ [0.9ex]\hdashline \\
     $f_{\rm sat}$ & fraction of satellite galaxy hosting QSO. only used for ``enforced" model. & 0-1  \\ [0.9ex] \\
     \bottomrule 
    \end{tabular}
    \label{tab:par-mcmc}
\end{table}

We describe details of how we fit the model parameters and generate predictions for the auto and cross-correlations in this section.

We use Multi-Tracer HOD ({\it hereafter} \mthod) mock catalogue developed in \textcolor{red}{Alam et. al. in prep.} to model the QSO. We take all the LRG and ELG galaxy in \mthod mock catalog with the information about host halo mass and whether it is central or satellite. The clustering properties and the number fraction with over-density environment matches very well between these mocks and eBOSS data. In principle one could as well model the magnitude of these galaxy and develop more complete model of QSO but that aspect is left for future study. The \mthod  mock catalog is created using publicly available MultiDark Planck (MPDL2) simulation \cite{2012MNRAS.423.3018P} through CosmoSim database \footnote{\url{https://www.cosmosim.org/cms/simulations/mdpl2/}}.
It is a dark matter only N-body simulation run using Adaptive-Refinement-Tree (ART) \citet{1997ApJS..111...73K}. MDPL2 assumes Flat $\Lambda$CDM cosmology with $\Omega_m=0.307$, $\Omega_b=0.048$, $h=0.67$, $n_s=0.96$ and $\sigma_8=0.82$. It is in a periodic box of side length 1000$\mpcoh$  and $3840^3$ particles. A halo catalogue using ROCKSTAR\footnote{\url{https://bitbucket.org/gfcstanford/rockstar}} halo finder \citet{behroozi13} was constructed using snapshot at effective redshift of $z = 0.86$ for MDPL2. We refer reader to \textcolor{red}{Alam et. al.} for the full details of simulation and how the \mthod is constructed.


The only question one would need to answer to obtain a QSO catalogue is that what is the probability for a galaxy's central balck hole to turn-on and become QSO instantaneously given galaxy properties. This turn-on probability is modelled using equation \ref{eq:turn-on}, which depends on halo mass, host galaxy type and whether its a satellite galaxy or not. The full list of parameters in our model is given in table \ref{tab:par-mcmc}. We have all together 9 parameters in ``inherent" model with 8 of them to model the halo mass dependence of $f_{\rm on}$ using linear spline with 8 knots listed in table \ref{tab:par-model} and the 9th parameter is to model fraction of QSO with host galaxy as LRG ($f_{\rm LRG}$). The ``enforced" model has and additional 10th parameter to model fraction of QSO in satellite galaxy $f_{\rm sat}$.

We perform Markov chain Monte Carlo (MCMC) analysis using emcee\citep{2013PASP..125..306F}. emcee is an efficient affine-invariant ensemble sampler. Therefore with emcee we sample the 9 or 10 parameter depending on the model. For any point in the parameter space one can evaluate the probability of a galaxy to turn-on using equation \ref{eq:turn-on} and hence obtain as sample of QSO in \mthod catalogue. We then evaluate the auto-correlation of QSO and its cross-correlation with LRG and ELG sample using methods decribed in section \ref{sec:measurement}. This measurement require pair-counting which needs to be performed at each step in of sampling. Therefore we use publicly available corrfunc \citep{manodeep_sinha_2016_55161} to evaluate pair-counts efficiently at each iteration. We have also precomputed the over-density field for galaxy in the \mthod catalogue using method described in \cite{2019MNRAS.483.4501A} which is then used to evaluate fraction of QSO as the function of over-density environment. Finally we evaluate $\chi^2$ for using following equation.

\begin{align}
    \chi^2 (\theta) & = (\vec{D}-\vec{M}(\theta)) \, C^{-1}(\vec{D}-\vec{M}(\theta))^T \\
    \vec{D} &=[w_p^{q}(r_p),w_p^{qL}(r_p),w_p^{qE}(r_p),f_q(\delta)] \\
    \vec{M}(\theta) &=[w_p^{q}(r_p,\theta),w_p^{qL}(r_p,\theta),w_p^{qE}(r_p,\theta),f_Q(\delta)]
    \label{eq:chi2}
\end{align}

where $w_p^{q}(r_p),w_p^{qL}(r_p),w_p^{qE}(r_p),f_q(\delta)$ represents the QSO auto, QSO$\times$LRG, QSO$\times$ELG and QSO fraction respectively. $\theta$ represents sampling parameters and $C^{-1}$ is the inverse covariance matrix obtained from jackknife analysis. The data and model is denoted by $\vec{D},\vec{M}(\theta)$ respectively. The MCMC process then sample the parameters according to the $\chi^2$ given by the model.

==> Tex/model.tex <==
\section{Modelling the QSO population}
\label{sec:model}


\begin{table*}
    \centering
    \caption{\sout{Describe the} Parameters of QSO turn-on models}
    \begin{tabular}{p{1.2cm} p{10cm} p{2.5cm}} \hline\hline
    {\bf Parameters} &  {\bf Description} & {\bf model} \\ [0.5ex] \hline\hline
      $f_{\rm on}(M_{\rm halo})$ &  {\rm This models the probability of galaxy to turn-on with given host halo mass. This is modeled as linear spline with 8 knots at location}  & All models\\
      & $\log_{10}(M_{\rm knots})=\left[11.2, 11.8, 12.15, 12.5, 12.75, 13.0, 13.5, 15.2\right]$ & \\ [0.9ex]\hdashline \\
      & Probability of galaxy to turn into QSO given its host galaxy type & All models \\
     G_{\rm type} &$\begin{array} {lcl} p(G_{\rm type}= {\rm LRG})  & = & f_{\rm LRG} \\ p(G_{\rm type}= {\rm ELG}) & = & 1-f_{\rm LRG} \end{array}$ & \\ [0.9ex]\hdashline \\
     & Probability of galaxy to turn into QSO given its host galaxy position &   \\
     G_{\rm pos} &$\begin{array} {lcl} p(G_{\rm pos}= {\rm satellite})  & = & f_{\rm sat} \\ p(G_{\rm pos}= {\rm central}) & = & 1-f_{\rm sat} \end{array}$ & Only for model with enforced $f_{\rm sat}$\\
     \bottomrule 
     \hline\hline
    \end{tabular}
    \label{tab:par-model}
\end{table*}


The basic idea for modelling QSO population used in this paper is that active \sout{galaxy} \sarah{galactic} nuclei (AGN) observed as QSO are not special in their host galaxy but a sub-sample of inherent galaxy population. Therefore, if one have a robust model of galaxy population in the same space and time where the target QSOs are living then one can simply model where QSO should turn-on. In principle one can imagine QSOs turn-on probability depends on the host galaxy properties and its black-hole mass strongly and not so much on the larger scale dark matter distribution or dark matter haloes. But, observational selection might imply one is selecting bright objects which are living in massive halo in which case for the observed sample the turn-on probability may depend on the host galaxy halo mass. But there are also hypothesis that QSO might live in special haloes and hence the turn-on  probability has narrow distribution with halo mass. In order to have minimal assumption the basic ingredient of our model is the turn-on probability of QSO from the parent galaxy population as halo mass. We first start with Multi-tracer HOD catalogue of ELG and LRG sample created by \textcolor{red}{Alam et. al. in prep.}. We suggest reader to look at \textcolor{red}{Alam et. al. in prep.} for details of MTHOD. In this mock catalogue we have measurement galaxy \sarah{is this measurements for galaxies? } with properties such as type between LRG and ELG and position in halo in terms of central and satellites \sarah{a clarification is needed here}. We argue \sarah{that} given the depth of galaxy sample\sarah{,} this should contain most \textcolor{red}{what fraction, how to asses?} of the QSO host galaxy. Therefore in order to obtain QSO sample we simply have to model the turn-on probability for galaxy in this simulated catalogue. We model the $f_{\rm on}(M_{\rm halo})$ with linear spline sampling 8 points between halo mass of $10^{11}\msolaroh$ and $10^{15}\msolaroh$. The model simply take the $f_{\rm on}$ with halo mass and sample galaxy to turn-on QSO following this distribution and the constrain on number density of QSO which is $2 \times 10^{-5}$. Once we have simulated QSO catalogue we can predict the projected auto correlation of QSO as well as cross correlation of QSO with LRG and ELG. Given the denser galaxy population one can also measure fraction of QSO as the function of over-density. Therefore we use these four measurement to constrain the parameters of the model. 

Once we have described the turn-on probability of QSO as the function of halo mass the next question one would face is whether this should depend on the type of host galaxy. In a model where the QSO turn-on probability is independent of type of host galaxy the fraction of QSO with a given type og host galaxy should be same as fraction of the host galaxy type in the parent population. We introduce a parameter $f_{\rm LRG}$ to define the fraction of QSO with host galaxy as LRG in the sample. Note that  $f_{\rm LRG}=0$ will mean that only ELG can turn-on to become QSO and $f_{\rm LRG}=1$ means only LRG can turn on to become QSO. If the posterior likelihood of either of these extreme becomes zeros then we can rule our QSO being turned-on in only one type of galaxy.

The last question one might ask is whether the QSO turn-on probability should be equal for galaxies which are central to the halo and the one which are satellite. \textcolor{red}{cite any literature which discusses whether it should depend on central /satellite}. We adopt two \sout{kind of} models to \sout{understand} study this aspect of QSO physics. In the first model, we \sout{say} \sarah{} that the \sout{ QSO turn-on probability doesn't} \sarah{the probability of a quasar to start activate} depend on whether the host galaxy is central or satellite. Therefore, the fraction of QSO hosted by satellite galaxy will be same as fraction of satellite galaxy in the parent population. We call this model has ``inherent satellite fraction'' and hence labelled ``$f_{\rm sat} \, (\rm inherent)$". \sout{On the other hand} In second model, we \sout{say} \sarah{assume} that QSO turn-on probability can depend on the whether the host galaxy is satellite or central and this is denoted by an additional parameter $f_{\rm sat}$ to denoted the probability of a QSO \sarah{to become active} with the host galaxy being central \sout{of} \sarah{or} satellite. This model allows extra degree of freedom where the satellite fraction in QSO population does not have to represent the satellite fraction of its parent galaxy population \sout{ but rather QSO can choose to only populate in central galaxy with $f_{\rm sat}=0$ and only in satellite galaxy by $f_{\rm sat}=1$} \sarah{}.

Finally the probability of a galaxy to turn-on and become QSO depends on its host halo mass ($M_{\rm halo}$), its galaxy type $(G_{\rm type}=\left[ {\rm LRG,ELG} \right])$ and its position in terms $(G_{\rm pos}=\left[ {\rm central,satellite} \right])$ and given by following equation.

\begin{equation}
    P_{\rm on}(M_{\rm halo},G_{\rm type},G_{\rm pos})= f_{\rm on}(M_{\rm halo}) p(G_{\rm type})p(G_{\rm pos})
    \label{eq:turn-on}
\end{equation}

where the details of different components in the above equation is described in table \ref{tab:par-model}. We note that here we consider the three probability to be independent of each other. It will be interesting to ask whether probability of QSO turn-on for host galaxy type and position are independent \textcolor{red}{ discuss some literature aspect here}. We consider more complicated model such that one has to consider joint probability of turn-on with host galaxy type and position is out of scope for this study and will be left for future work. Given the limitation of our current measurement especially lack of information at small scale due to fibre collision we do not expect this assumption to affect our conclusion in qualitative sense.


%Generally, it is considered that most QSO's are central because clustering of QSO in one-halo regime show no-significant extra power on top of two-halo term. Such study will imply that QSO's are preferentially turned-on in central galaxy because satellite fraction of parent galaxy population is typically of the order of $10-20\%$. Therefore, one can argue that we need additional degree of freedom in our model to allow central galaxy to preferentially turn-on compared to satellite galaxy. Therefore we introduce and additional parameter $f_{\rm sat}$ in our model which essential say that what  fraction of QSO must be satellite and then turn-on central and satellite galaxies given $f_{\rm on}(M_{\rm halo})$ and respecting satellite fraction.  

